Evaluation of an Autonomous Surface Robot Equipped with a Transformable Mobility Mechanism for Efficient Mobility Control

Efficient mobility and power consumption are critical for autonomous water surface robots in long-term water environmental monitoring. This study develops and evaluates a transformable mobility mechanism for a water surface robot with two control modes: station-keeping and traveling to improve energy efficiency and maneuverability. Field experiments show that, in a round-trip task between two points, the traveling mode reduces power consumption by 10\% and decreases the total time required for travel by 5\% compared to the station-keeping mode. These results confirm the effectiveness of the transformable mobility mechanism for enhancing operational efficiency in patrolling on water surface.

==> allocation.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{thruster_allocation.jpg}
    \caption{Thruster allocation}
    \label{fig:allocation}
\end{figure}


==> coordinate.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{coordinate.jpg}
    \caption{Coordinate system}
    \label{fig:coordinate}
\end{figure}


==> exp_field.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{exp_field.jpg}
    \caption{Experimental field}
    \label{fig:exp_field}
\end{figure}


==> keep.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{keep.jpg}
    \caption{Keeping mode}
    \label{fig:keep}
\end{figure}


==> straight.tex <==
\begin{figure}[htb]
  \centering
    \includegraphics[width=\linewidth]{straight.jpg}
    \caption{Straight mode}
    \label{fig:straight}
\end{figure}

